Locality Matters: A Scalable Value Decomposition Approach for Cooperative Multi-Agent Reinforcement Learning

Cooperative multi-agent reinforcement learning (MARL) faces significant scalability issues due to state and action spaces that are exponentially large in the number of agents. As environments grow in size, effective credit assignment becomes increasingly harder and often results in infeasible learning times. Still, in many real-world settings, there exist simplified underlying dynamics that can be leveraged for more scalable solutions. In this work, we exploit such locality structures effectively whilst maintaining global cooperation. We propose a novel, value-based multi-agent algorithm called LOMAQ, which incorporates local rewards in the Centralized Training Decentralized Execution paradigm. Additionally, we provide a direct reward decomposition method for finding these local rewards when only a global signal is provided. We test our method empirically, showing it scales well compared to other methods, significantly improving performance and convergence speed.

==> comments.tex <==
% We denote by $\T$ the set of all possible histories and define the (history dependent) policy of agent $i$ as a mapping ${\pi_i: \T \times \A \mapsto [0,1]}$ such that $\pi_i(a | \tau_t)$ is the probability that agent $i$ will choose action $a_t = a$ given history $\tau_t = (s_0, a_0, \hdots, s_t)$. 



% \begin{definition}[Partitioned rewards]
% \label{def:additive1}
% If $\p$ is some partition of $\V$, and $\brk[c]*{r_i}_{i=1}^n$ is some reward decomposition, then we define the induced \emph{partitioned rewards} $r_J$ such that:

% \begin{align*}
%     \forall J \in \p:
%      r_J(s, a) = \sum_{i \in J} r_i(s_i, a_i)
% \end{align*}
% \end{definition}

% We note that for $\beta=1$, \Cref{def:additive2} returns the additively decomposable reward of \Cref{def:additive1}. 

% We offer a refinement to Definition~\ref{def:additive2} by introducing another parameter $l$, which will define the largest number of agents in the agent neighborhood that the local reward functions can depend on. Denoting $r_B = \sum_{i \in B} r_i$ for some set $B \subseteq \V$, we have the following definition.

% \begin{definition}[Additively decomposable reward by ($\beta$, $l$)]
% \label{definition: additive3}
% We say a reward function $r(s, a)$ additively decomposable by ($\beta$, $l$) if there exist $r_{n_j}(s_{n_j}, a_{n_j})$ such that for every $s \in S$, $a \in A$, 

% \[
% N(\beta, l) = 
% \left\{
% n_j | 
% \exists i \in n_j: 
% n_j \in N^{\beta}_i, 
% n_j \textrm{ is a s.c.c},
% |n_j| \leq l
% \right\}
% \]

% \[
%  r(s, a) = \sum_{n_j \in N(\beta, l)}r_{n_j}(s_{n_j}, a_{n_j})
% \]
% \end{definition}

% % Note that if parameter $l \geq \max_{i} \{|N^{\beta}_i|\}$, then Definition~\ref{def:additive2} and Definition~\ref{def:additive3} are equivalent, since every agents reward can be decomposed into a reward function that is dependent on the entire $\beta$-neighborhood that can contain all the sub-functions. Note that setting $\beta \geq \text{diam}(G)$ leads us to a decomposition of $\sum^l_{i=1}{n \choose i}$ local reward functions that completely disregards the graph structure. 

% \Cref{definition: additive3} extends the commonly used assumption of decomposing the reward into small groups of agents, but enforces the connectivity of these groups in the dependency graph. For example, if $\beta=1$ and $l=2$, then we get a pairwise-decomposition of the reward function for all agents that are directly connected in $\G$. 

% Also note that Definition~\ref{def:additive3} differs from the previous definitions due to the number of reward functions it may contain, which can be much larger than ${n}$. This motivates us to create a mapping between the local reward functions and the agents, such that every local reward function $r_{n_j}$ is mapped to agent $i$ if $i \in n_j$. this mapping can be thought of as "Every local reward function $r_{n_j}$ that ties directly to agent $i$". 

% The learned rewards for this case don't just expedite learning, they're also exlpainable



% \roy{
% Guy tell me what you think:
% 1) General Experiments of LOMA$Q$ with comparisons to state of the art
% 2) Experiments with a lot of agents to show scalability
% 3) Experiments that show the dependency on $\kappa$, and image that shows non-cooperation for $\kappa=0$ (local IQL)
% 4) Experiments that compare results with reward decomposition and without
% 5) General reward decomposition visualizations with 1 and 2 agents, with and without regularization
% 6) Maybe an experiment where reward decomposition with a star shape is favored over a global reward
% }


% \subsubsection{Reward decompositions} We also test LOMA$Q$ with different reward decompositions, varying in size of $n_j$. We use the environment local reward signals $r_i$, and evenly distribute them between agents in $N_i^{z}$ with increasing $z$ These results can be seen in \Cref{fig:changing_reward}.

% \begin{figure}[t!]
% \centering
% \includegraphics[width=0.5\columnwidth]{results/glocal_rewards.png}
% \caption{Return mean for changing reward decompositions}
% \label{fig:changing_reward}
% \end{figure}


% The VDN approximation is closely related to the decoupled case shown in \Cref{proposition: decoupled case}. If the VDN approximation holds exactly, i.e. $Q(s, a) = \sum_{i=1}^n U_i(s_i, a_i)$, then it satisfies \Cref{definition: qsm} with $\p= \brk[c]*{\brk[c]*{1}, \brk[c]*{2}, \hdots, \brk[c]*{n}}$ by a similar argument. This means that if $\M$ is representable by VDN, it is representable by LOMA$Q$ for any partition $\p$. In practice, both methods attempt to approximate the $Q$ values in different manners, so results may differ between these cases.


% \begin{align*}
%     \forall J \in \p:
%     r_{c_J}(s, a) = \sum_{j \in J} r_j(s, a)
% \end{align*}




% The following proposition suggests another expressibility trade-off for \Cref{assumption: monotonic utilities}, controlled this time by the locality of rewards.

% \begin{restatable}{proposition}{rewardrefinement}
%     Let $\M = (\G, \s, \A, P, r, \gamma)$, and let $\brk[c]*{r_i(s_i, a_i)}_{i=1}^n$, $\brk[c]*{r_i'(s, a)}_{i=1}^n$
%     be some decompositions of $r$. Assume that $\Cref{assumption: monotonic utilities}$ holds with $\p$, $\brk[c]*{r_i}_{i=1}^n$. If $r_i' = \sum_{j = 1}^n \alpha_{i, j} r_j$ and $\alpha_{i, j} \geq 0$, then $\Cref{assumption: monotonic utilities}$ holds with $\p$ for $\brk[c]*{r_i'}_{i=1}^n$ as well.
% \end{restatable}


% \rewardrefinement*
% \begin{proof}

% Let $\brk[c]*{r_i(s_i, a_i)}_{i=1}^n$, $\brk[c]*{r_i'(s, a)}_{i=1}^n$ be such decompositions. We denote $\brk[c]*{{F}_{J}^\pi}_{J \in \p}$, $\brk[c]*{{U}_i^\pi}_{i \in \V}$ as the functions that satisfy \Cref{assumption: monotonic utilities} for $\brk[c]*{r_i(s_i, a_i)}_{i=1}^n$. Due to the linearity of expectation we get:

% \begin{align*}
%     {Q'}_i^\pi(s,a)
%     & = \expect*{\pi}{
%         \sum_{t=0}^\infty \gamma^t r'_i(s(t), a(t)) | s(0) = s, a(0) = a
%     } \\
%     & = \expect*{\pi}{
%         \sum_{t=0}^\infty \gamma^t \brk[r]*{
%             \alpha_{i, j}\sum_{j \in \V} r_j(s(t), a(t))
%         }
%         | s(0) = s, a(0) = a
%     } \\
%     & = \alpha_{i, j} \sum_{j \in \V} \brk[r]*{
%         \expect*{\pi}{
%             \sum_{t=0}^\infty \gamma^t r_j(s(t), a(t)) | s(0) = s, a(0) = a
%         }
%     } \\
%     & = \sum_{j \in \V} \alpha_{i, j} Q_j^\pi(s,a)
% \end{align*}

% We now define $\brk[c]*{{F'}_{J}^\pi}_{J \in \p}$, $\brk[c]*{{U'}_i^\pi}_{i \in \V}$ for the new reward decomposition. By setting the utilities to be identical to the original utilities ${U'}_i^\pi = U_i^\pi$, we get:

% \begin{align*}
%     \forall J \in \p:
%     {F'}_J^\pi(\mathbf{U}(s,a))
%     & = \sum_{i \in J} {Q'}_i^\pi(s,a) \\
%     & = \sum_{i \in J}  \sum_{j \in V} \alpha_{i, j} Q_j^\pi(s,a) \\
%     & = \sum_{i \in J} \frac{1}{|A(J')|}\sum_{j \in A(J')} Q_j^\pi(s,a) \\ 
%     & = \frac{|J|}{|A(J')|}\sum_{j \in A(J')} Q_j^\pi(s,a) \\
%     & = \frac{|J'|}{|A(J')|} F_{A(J')}
% \end{align*}

% Which therefore means:

% \begin{align*}
%     \nabla_{\mathbf{U}} {F'}_{J'}^\pi 
%     = \nabla_{\mathbf{U}} \brk[r]*{
%         \frac{|J'|}{|A(J')|} F_{A(J')}
%     } 
%     = \frac{|J'|}{|A(J')|} \nabla_{\mathbf{U}} F_{A(J')} \geq \mathbf{0}
% \end{align*}

% Therefore satisfying \Cref{assumption: monotonic utilities} with partition $\p'$ and reward decomposition $\brk[c]*{r_i'(s,a)}_{i=1}^n$.

    
% \end{proof}



% \subsection*{Derivatives of the Losses - OLD, not updated yet}

% We can compare the derivatives between the two losses. Let $\theta_{1i}$ denote the parameters of Agent $i$'s Utility Network, and $\theta_{2i}$ denote the parameters of the $i$'th Local Mixing Network. Therefore, we can deduce that:

% \guy{What are all these bold fonts? Looks strange}
% \[
% \pdv{L_1}{\theta_{1i}} = 
% -2 \pdv{U_i}{\theta_{1i}}
% \left(
% \sum_{j | i \in N^k_j}
% \pdv{Q_j}{U_i}
% \pmb{
% \left(
% \sum_{m=1}^{N}
% \left(
% y_m - Q_m^\theta(s, a)
% \right)
% \right)
% }
% \right)
% \]

% \[
% \pdv{L_2}{\theta_{1i}} = 
% -2 \pdv{U_i}{\theta_{1i}}
% \left(
% \sum_{j | i \in N^k_j}
% \pdv{Q_j}{U_i}
% \pmb{
% \left(
% y_i - Q_i^\theta(s, a)
% \right)
% }
% \right)
% \]

% \[
% \pdv{L_1}{\theta_{2i}} = 
% -2 \pdv{Q_i}{\theta_{2i}}
% \pmb{
% \left(
% \sum_{m=1}^{N}
% \left(
% y_m - Q_m^\theta(s, a)
% \right)
% \right)
% }
% \]

% \[
% \pdv{L_2}{\theta_{2i}} = 
% -2 \pdv{Q_i}{\theta_{2i}}
% \pmb{
% \left(
% y_i - Q_i^\theta(s, a)
% \right)
% }
% \]

% \noindent Where the changes between derivatives in bold. We can see from this example that the derivatives are also quite similar, besides the fact that all the agents $L_1$ TD-errors are used to compute each gradient, whereas $L_2$ is only dependent on $i$ . (NEEDS WORK + more explaining)

% \noindent We can see that for $z=0$ we get the derivative of $L_2$, and for $z \geq n$ we get $nL_1$.

% \[
% \pdv{L_z}{\theta_{2i}} = 
% -2 \pdv{Q_i}{\theta_{2i}}
% \pmb{
% \left(
% \sum_{j | j \in N^z_i}
% \left(
% \sum_{m | m \in N^z_j}
% \left(
% y_m - Q_m^\theta(s, a)
% \right)
% \right)
% \right)
% }
% \]

% \noindent We can see that for $z=0$ we get the derivative of $\pdv{L_2}{\theta_{2i}}$, and for $z \geq n$ we get the derivative of $n\pdv{L_1}{\theta_{2i}}$. (NEEDS MORE + testing)



% \subsubsection{LOMA$Q$} Our main method of enforcing monotinicity is a regularization technique, which penalizes negative derivatives of $F_J$ w.r.t $U_i$ for every $J \in \p$. Our method assumes that $\p_{\text{approx}}$ is a refinement of $\p_{\text{enforce}}$. 

% Let $\brk[c]*{i_J}_{J \in \p_{\text{enforce}}} \subseteq [|\p_{\text{enforce}}|]$ be some ordering of $\p_{\text{enforce}}$. We define $\vec{f}^{\theta}: \R^{n} \mapsto \R^{|\p_{\text{enforce}}|}$, such that $\vec{f}_{i_J}^{\theta} = F_J^{\theta}(\mathbf{U}^\theta)$. Let $\J$ denote the jacobian of $\vec{f}$. \guy{Just use $\nabla$} Our regularization loss is therefore:

% \begin{align*}
%     \mathcal{R}_{reg} = 
%     \lambda_{\text{reg}} \sum_{i=1}^n \sum_{j=1}^{|\p_{\text{enforce}}|} \text{Relu}(-\J_{ij}) 
% \end{align*}
% \guy{Don't write the regularization this way. RELU is an activation function. Write instead a formal regularization over the set of positive jacobians, and then say that in practice we do this using a Relu activation, and write the loss.}

% Where $\lambda_{\text{reg}}$ is a regularization weighting hyperparameter. By penalizing these negative derivatives, we softly enforce \Cref{assumption: monotonic utilities} for $\p_{\text{enforce}}$. Particularly for $\p_{\text{enforce}} = \{\V\}$, LOMA$Q$ enforces the non-negativity of $\nabla Q^{\theta}$, as done in $Q$-mix using non-negative weights for $Q^{\theta}$.

% \subsubsection{LOMA$Q$-h (LOMA$Q$-hard)} We offer a second method for enforcing monotonicity, by extending the technique used in $Q$-mix \guy{Again with the Qmix}. Firstly, we assert $\p_{\text{enforce}} = \p_{\text{approx}}$ \guy{I still don't understand what $\p_{\text{approx}}$ is. Please add a pseudocode algorithm}. We then enforce non-negative weights in every $\theta$ using hypernetworks. Similarly, we input the global state to these hypernetworks, since every $F_J$ is allowed to depend on the extra state information in non-monotonic ways.


